PureGen: Universal Data Purification for Train-Time Poison Defense via Generative Model Dynamics

Train-time data poisoning attacks threaten machine learning models by introducing adversarial examples during training, leading to misclassification. Current defense methods often reduce generalization performance, are attack-specific, and impose significant training overhead. To address this, we introduce a set of universal data purification methods using a stochastic transform, $\Psi(x)$, realized via iterative Langevin dynamics of Energy-Based Models (EBMs), Denoising Diffusion Probabilistic Models (DDPMs), or both. These approaches purify poisoned data with minimal impact on classifier generalization. Our specially trained EBMs and DDPMs provide state-of-the-art defense against various attacks (including Narcissus, Bullseye Polytope, Gradient Matching) on CIFAR-10, Tiny-ImageNet, and CINIC-10, without needing attack or classifier-specific information. We discuss performance trade-offs and show that our methods remain highly effective even with poisoned or distributionally shifted generative model training data.

==> PureGenDefense/Algos/train_clf.tex <==
\begin{algorithmic}
\REQUIRE Train dataset $X$, Model $F_\phi$, LR $\eta_{opt}$ %, Epochs $T$ 
\ENSURE Pre-process dataset via MCMC: $\Tilde{X}\gets\Psi_{T}(X)$
\STATE Initialize weights $\phi_1$ for Classifier $F$
\WHILE{$\phi_i$ not converged}
    \STATE $i \gets i + 1$\\ 
    \FOR{$\Tilde{x} \in \Tilde{X}$}
        \STATE Calculate the Grads and Update Params
        \STATE $\mathfrak{g}_i \gets \nabla_{\phi}F_{\phi_{i-1}}(\Tilde{x}_i)$
        \STATE $\phi_i \gets \phi_{t-1} - \eta_{opt} \mathfrak{g}_t$ 
    \ENDFOR
\ENDWHILE
\end{algorithmic}
% \begin{algorithmic}
   % \REQUIRE {Train dataset $X$, Model $f_\theta$, LR $\eta_{opt}$, $\lambda$, small number $T$}
   %  \FOR{$i = 1 \to T$}
   %      \STATE $\theta^i = \theta^{i-1} - \eta \nabla_{\theta} L(\theta^{i-1}, X)$ \Comment{Train the model for a few epochs}
   %  \ENDFOR
% \end{algorithmic}




==> PureGenDefense/Algos/train_ebm.tex <==
\begin{algorithmic}
\REQUIRE ConvNet potential $U(x; \theta)$, images $x^+_i \in  \mathcal{X} or (\mathcal{X} \setminus \mathcal{P}_{all})$, Langevin steps $K=100$, temp $\tau=1e-4$, image bank $\{ Y \}_{i=1}^{1250}$
\ENSURE Weights $\theta_{J+1}$ for $U(x ; \theta)$
\STATE Initialize image bank $\{ Y \}_{i=1}^s$ with $s=1250$ images
\FOR{$j$ in iters}
    \STATE Draw batch $\{x_{(i)}^+\}_{i=1}^m$; initial negatives $\{ Y_i^{(0)} \}_{i=1}^m$ from $\{ Y \}$
    \STATE Update $\{ Y_i^{(0)} \}$ using Langevin dynamics:
        \[ Y^{(k)}_i = Y^{(k-1)}_i - \frac{\tau^2}{2} \nabla_y U(Y^{(k-1)}_i ; \theta_j) + \tau Z_{i, k} \]
    \STATE Update image bank $\{ Y_i^{(K)} \}_{i=1}^m$; weights $\theta_{j+1}$ using:
        \[ \Delta \theta_j= \nabla_\theta \left( \frac{1}{n} \sum_{i=1}^n U(X^+_i ; \theta_j) - \frac{1}{m}\sum_{i=1}^m U(X_i^-; \theta_j) \right) \]
\ENDFOR
\end{algorithmic}

==> PureGenDefense/Tables/full_core_scratch.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}rcccccccccc@{}}
\toprule
\multicolumn{11}{c}{\textbf{From Scratch}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \midrule
\textbf{}                                                            & \multicolumn{5}{c}{\textbf{200 - Epochs}}                                                                                                                                                                                                                                                                                               & \multicolumn{5}{c}{\textbf{80 - Epochs}}                                                                                                                                                                                                                                                                                                \\ \cmidrule(lr){2-6} \cmidrule(lr){7-11} 
\textbf{}                                                            & \multicolumn{2}{c}{\textbf{Gradient Matching-1\%}}                                                                              & \multicolumn{3}{c}{\textbf{Narcissus-1\%}}                                                                                                                                                            & \multicolumn{2}{c}{\textbf{Gradient Matching-1\%}}                                                                              & \multicolumn{3}{c}{\textbf{Narcissus-1\%}}                                                                                                                                                            \\ \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-11} 
\textbf{}                                                            & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max Poison \\ Success (\%) ↓\end{tabular} \\ \midrule
\multicolumn{1}{l|}{None}                                            & 44.00                                                     & 94.84$_{0.2}$                                                       & 43.95$_{33.6}$                                                    & 94.89$_{0.2}$                                                       & 93.59                                                         & 47.00                                                     & 93.79$_{0.2}$                                                       & 32.51$_{30.3}$                                                    & 93.76$_{0.2}$                                                       & 79.43                                                         \\
\multicolumn{1}{l|}{\epic-0.1*}                       & 34.00                                                     & 91.27$_{0.4}$                                                       & 30.18$_{32.2}$                                                    & 91.17$_{0.2}$                                                       & 81.50                                                         & 27.00                                                     & 90.87$_{0.4}$                                                       & 24.15$_{30.1}$                                                    & 90.92$_{0.4}$                                                       & 79.42                                                         \\
\multicolumn{1}{l|}{\epic-0.2}                        & 21.00                                                     & 88.04$_{0.7}$                                                       & 32.50$_{33.5}$                                                    & 86.89$_{0.5}$                                                       & 84.39                                                         & 28.00                                                     & 91.02$_{0.4}$                                                       & 23.75$_{29.2}$                                                    & 89.72$_{0.3}$                                                       & 74.28                                                         \\
\multicolumn{1}{l|}{\epic-0.3*}                       & 10.00                                                     & 85.14$_{1.2}$                                                       & 27.31$_{34.0}$                                                    & 82.20$_{1.1}$                                                       & 84.71                                                         & 44.00                                                     & 92.46$_{0.3}$                                                       & 21.53$_{28.8}$                                                    & 88.05$_{1.1}$                                                       & 80.75                                                         \\
\multicolumn{1}{l|}{\epic$_{reported}$}                       & 1.00                                                     & 90.26                                                       & NA                                                    & NA                                                      & NA                                                         & NA                                                     & NA                                                       & NA                                                    & NA                                                       & NA                                                        \\
\multicolumn{1}{l|}{\friends-B}                       & 1.00                                                      & \textbf{91.16$_{0.4}$}                                              & 8.32$_{22.3}$                                                     & 91.01$_{0.4}$                                                       & 71.76                                                         & 2.00                                                      & 90.07$_{0.4}$                                                       & \textbf{1.42$_{0.8}$}                                             & 90.06$_{0.3}$                                                       & 2.77                                                          \\
\multicolumn{1}{l|}{\friends-G*}                      & \textbf{0.00}                                             & \textbf{91.15$_{0.4}$}                                               & 9.49$_{25.9}$                                                     & 91.06$_{0.2}$                                                       & 83.03                                                         & \textbf{1.00}                                             & 90.09$_{0.4}$                                                       & \textbf{1.37$_{0.9}$}                                              & 90.01$_{0.2}$                                                       & 3.18                                                          \\ \midrule
\multicolumn{1}{l|}{\textbf{\pgenEBM}}                   & \textbf{0.00}                                             & \textbf{92.26$_{0.2}$}                                               & \textbf{1.27$_{0.6}$}                                              & \textbf{92.91$_{0.2}$}                                               & \textbf{2.16}                                                 & \textbf{1.00}                                             & \textbf{91.36$_{0.3}$}                                               & \textbf{1.46$_{0.8}$}                                              & \textbf{91.83$_{0.3}$}                                               & \textbf{2.49}                                                 \\
\multicolumn{1}{l|}{\textbf{\pgenEBM-P}}                 & NA                                                          & NA                                                                & \textbf{1.38$_{0.7}$}                                              & \textbf{92.70$_{0.2}$}                                               & \textbf{2.78}                                                 & NA                                                          & NA                                                                & \textbf{1.63$_{1.0}$}                                              & \textbf{91.49$_{0.3}$}                                               & 3.47                                                          \\
\multicolumn{1}{l|}{\textbf{\pgenEBM$_{CN-10}$}}          & \textbf{0.00}                                             & \textbf{92.99$_{0.2}$}                                               & \textbf{1.43$_{0.8}$}                                              & \textbf{92.90$_{0.2}$}                                               & \textbf{3.06}                                                 & \textbf{1.00}                                             & \textbf{92.02$_{0.2}$}                                               & \textbf{1.50$_{0.9}$}                                              & \textbf{92.03$_{0.2}$}                                               & \textbf{2.52}                                                 \\
\multicolumn{1}{l|}{\textbf{\pgenEBM$_{IN}$}} & 1.00                                                      & \textbf{92.98$_{0.2}$}                                               & \textbf{1.39$_{0.8}$}                                              & \textbf{92.92$_{0.2}$}                                               & \textbf{2.50}                                                 & \textbf{1.00}                                             & \textbf{92.02$_{0.2}$}                                               & \textbf{1.52$_{0.8}$}                                              & \textbf{92.02$_{0.3}$}                                               & \textbf{2.81}                                                 \\
\multicolumn{1}{l|}{\textbf{\pgenEBM-P$_{CN-10}$}}       & NA                                                          & NA                                                                & \textbf{1.64$_{0.01}$}                                             & \textbf{92.86$_{0.20}$}                                              & \textbf{4.34}                                                 & NA                                                          & NA                                                                & \textbf{1.68$_{1.0}$}                                              & \textbf{92.07$_{0.2}$}                                               & 3.34                                                          \\ \bottomrule
\end{tabular}


==> PureGenDefense/Tables/full_core_transfer.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}rccccccccc@{}}
\toprule
\multicolumn{10}{c}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \midrule
\textbf{}                                                   & \multicolumn{5}{c}{\textbf{Fine-Tune}}                                                                                                                                                                                                                                                                                                  & \multicolumn{4}{c}{\textbf{Linear - Bullseye Polytope}}                                                                                                                                                                                                           \\ \cmidrule(lr){2-6} \cmidrule(lr){7-10}
\textbf{}                                                   & \multicolumn{2}{c}{\textbf{Bullseye Polytope-10\%}}                                                                             & \multicolumn{3}{c}{\textbf{Narcissus-10\%}}                                                                                                                                                           & \multicolumn{2}{c}{\textbf{BlackBox-10\%}}                                                                                      & \multicolumn{2}{c}{\textbf{WhiteBox-1\%}}                                                                                       \\ \cmidrule(lr){2-3} \cmidrule(lr){4-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10}
\textbf{}                                                   & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} \\ \midrule
\multicolumn{1}{l|}{None}                                   & 46.00                                                     & 89.84$_{0.9}$                                                       & 33.41$_{33.9}$                                                    & 90.14$_{2.4}$                                                       & 98.27                                                         & 93.75                                                     & 83.59$_{2.4}$                                                       & 98.00                                                     & 70.09$_{0.2}$                                                       \\
\multicolumn{1}{l|}{\epic-0.1}               & 50.00                                                     & 89.00$_{1.8}$                                                       & 32.40$_{33.7}$                                                    & 90.02$_{2.2}$                                                       & 98.95                                                         & 91.67                                                     & 83.48$_{2.9}$                                                       & 98.00                                                     & 69.35$_{0.3}$                                                       \\
\multicolumn{1}{l|}{\epic-0.2*}              & 42.00                                                     & 81.95$_{5.6}$                                                       & 20.93$_{27.1}$                                                    & 88.58$_{2.0}$                                                       & 91.72                                                         & 66.67                                                     & 84.34$_{3.8}$                                                       & 91.00                                                     & 64.79$_{0.7}$                                                       \\
\multicolumn{1}{l|}{\epic-0.3}      & 44.00                                                     & 86.75$_{6.3}$                                                       & 28.01$_{34.9}$                                                    & 84.36$_{6.3}$                                                       & 99.91                                                         & 66.67                                                     & 83.23$_{3.8}$                                                       & 63.00                                                     & 60.86$_{1.5}$                                                       \\
\multicolumn{1}{l|}{\friends-B}              & 8.00                                                      & 87.80$_{1.1}$                                                       & 3.34$_{5.7}$                                                      & 89.62$_{0.5}$                                                       & 19.48                                                         & 35.42                                                     & 84.97$_{2.2}$                                                       & 19.00                                                     & 60.85$_{0.6}$                                                       \\
\multicolumn{1}{l|}{\friends-G*}             & 8.00                                                      & 87.82$_{1.2}$                                                       & 3.04$_{5.1}$                                                      & 89.81$_{0.5}$                                                       & 17.32                                                         & 33.33                                                     & 85.18$_{2.3}$                                                       & 19.00                                                     & 60.90$_{0.6}$                                                       \\ \midrule
\multicolumn{1}{l|}{\textbf{\pgenEBM}}          & \textbf{0.00}                                             & \textbf{88.95$_{1.1}$}                                              & \textbf{1.98$_{1.7}$}                                             & \textbf{91.40$_{0.4}$}                                              & \textbf{5.98}                                                 & \textbf{0.00}                                             & \textbf{92.89$_{0.2}$}                                              & \textbf{6.00}                                             & \textbf{64.51$_{0.6}$}                                              \\
\multicolumn{1}{l|}{\textbf{\pgenEBM-P}}        & NA                                                          & NA                                                                & \textbf{3.66$_{4.63}$}                                                    & \textbf{90.89$_{0.31}$}                                                       & 16.04                                                         & NA                                                          & NA                                                                & NA                                                          & NA                                                                \\
\multicolumn{1}{l|}{\textbf{\pgenEBM$_{CN-10}$}} & \textbf{0.00}                                             & \textbf{88.67$_{1.2}$}                                              & \textbf{2.97$_{2.5}$}                                             & \textbf{90.99$_{0.3}$}                                              & \textbf{7.95}                                                 & \textbf{0.00}                                             & \textbf{92.82$_{0.1}$}                                              & \textbf{6.00}                                             & \textbf{64.44$_{0.4}$}                                              \\
\multicolumn{1}{l|}{\textbf{\pgenEBM$_{IN}$}}             & \textbf{0.00}                                             & \textbf{87.52$_{1.2}$}                                              & \textbf{2.02$_{1.0}$}                                             & \textbf{89.78$_{0.6}$}                                              & \textbf{3.85}                                                 & \textbf{0.00}                                             & \textbf{92.38$_{0.3}$}                                              & \textbf{6.00}                                             & \textbf{64.98$_{0.3}$}                                              \\ \bottomrule
\end{tabular}

==> PureGenDefense/Tables/models_and_datasets.tex <==
\begin{tabular}{@{}lllll@{}}
\toprule
\multicolumn{5}{c}{\textbf{CINIC-10 Narcissus - 1\% From-Scratch (200 Epochs)}}                                                                                                                                                                                                                                                                                                                           \\ \midrule
                                             & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success (\%) ↓\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Avg Natural\\  Accuracy (\%) ↑\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Max Poison \\ Success (\%) ↓\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}CIFAR-10\\ Accuracy (\%) ↑\end{tabular}} \\ \midrule
\multicolumn{1}{l|}{None}                    & 62.06$_{0.21}$                                                                      & 86.32$_{0.10}$                                                                          & 90.79                                                                           & 94.22$_{0.16}$                                                                      \\
\multicolumn{1}{l|}{\epic}    & 49.50$_{0.27}$                                                                        & 81.91$_{0.08}$                                                                          & 91.35                                                                           & 91.10$_{0.21}$                                                                      \\
\multicolumn{1}{l|}{\friends} & 11.17$_{0.25}$                                                                        & 77.53$_{0.60}$                                                                          & 82.21                                                                           & 88.27$_{0.68}$                                                                      \\
\multicolumn{1}{l|}{\pebm}    & \textbf{7.73$_{0.08}$}                                                                & \textbf{82.37$_{0.14}$}                                                               & \textbf{29.48}                                                                  & \textbf{91.98$_{0.16}$}                                                           \\ \bottomrule
\toprule
                                        \multicolumn{5}{c}{\textbf{From Scratch NS-1\% (200 epochs)}}                                                                                                                                                                                                                     \\ \midrule
\textbf{}                                              & \multicolumn{2}{c}{\textbf{MobileNetV2}}                                                                                                   & \multicolumn{2}{c}{\textbf{DenseNet121}}                                                                                             \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
\textbf{}                                              & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success  (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular}       & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success  (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} \\ \midrule
\multicolumn{1}{l|}{None}                              & 32.70$_{0.25}$                                                     & 93.92$_{0.13}$                                             & 46.52$_{32.2}$                                                                        & 95.33$_{0.1}$                                                                                                             \\
\multicolumn{1}{l|}{\epic}              & 22.35$_{0.24}$                                                     & 78.16$_{9.93}$                                                            & 32.60$_{29.4}$                                                                        & 85.12$_{2.4}$                                                         \\
\multicolumn{1}{l|}{\friends}           & 2.00$_{0.01}$                                                      & 88.82$_{0.57}$                                                             & 8.60$_{21.2}$                                                                         & 91.55$_{0.3}$                                                           \\
\multicolumn{1}{l|}{\textbf{\pebm}}     & \textbf{1.64$_{0.01}$}                                             & \textbf{91.75$_{0.13}$}                                                   & \textbf{1.42$_{0.7}$}                                                                 & \textbf{93.48$_{0.1}$}                                                         \\ \midrule
                                      \multicolumn{5}{c}{\textbf{Linear Transfer  WhiteBox BP-10\%}}                                                                                                                                                                                                                    \\ \midrule
                                                       & \multicolumn{2}{c}{\textbf{MobileNetV2}}                                                                                                   & \multicolumn{2}{c}{\textbf{DenseNet121}}                                                                                             \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
                                                       & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular}       & \begin{tabular}[c]{@{}c@{}}Poison \\ Success (\%) ↓\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} \\ \midrule
\multicolumn{1}{l|}{None}                              & 81.25                                                          & 73.27$_{0.97}$                                                            & 73.47                                                          & 82.13$_{1.62}$                                                      \\
\multicolumn{1}{l|}{\epic}              & 56.25                                                          & 54.47$_{5.57}$                                                            & 66.67                                                          & 70.20$_{10.15}$                                                     \\
\multicolumn{1}{l|}{\friends}           & 41.67                                                          & 68.86$_{1.50}$                                                            & 60.42                                                          & 80.22$_{1.90}$                                                      \\
\multicolumn{1}{l|}{\textbf{\pebm}}     & \textbf{0.00}                                                  & \textbf{78.57$_{1.37}$}                                                   & \textbf{0.00}                                                  & \textbf{89.29$_{0.94}$}                                             \\ \midrule
      \multicolumn{5}{c}{\textbf{Hyperlight Bench CIFAR-10 NS-1\% (10 Epochs)}}                                                                                                                                                                                                         \\ \midrule
                                                       & \begin{tabular}[c]{@{}c@{}}Avg Poison \\ Success (\%) ↓\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg Nat \\ Acc (\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max Poison\\ Success (\%) ↓\end{tabular}   & \begin{tabular}[c]{@{}c@{}}Train Time (s) \\ (Epoch Time)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{None}                              & 76.39$_{16.35}$                                                  & 93.95$_{0.10}$                                                          & 95.69                                                            & 6.81$_{0.62}$ (0.68)                                                                  \\
\multicolumn{1}{l|}{\epic}              & 10.58$_{18.35}$                                                  & 24.88$_{6.04}$                                                          & 50.21                                                            & 612.43$_{30.16}$ (61.24)                                                              \\
\multicolumn{1}{l|}{\friends}           & 11.35$_{18.45}$                                                  & 87.03$_{1.52}$	                                                          & 56.65	                                                            & 427.50$_{0.50}$ (42.75)                                                                  \\
\multicolumn{1}{l|}{\textbf{\pebm-25}}  & 10.59$_{26.04}$                                                  & 92.75$_{0.13}$                                                          & 84.60                                                            & 54.70$_{0.48}$ (0.65)                                                                 \\
\multicolumn{1}{l|}{\textbf{\pebm-50}}  & \textbf{2.16$_{1.22}$}                                           & \textbf{92.38$_{0.17}$}                                                 & \textbf{3.74}                                                    & 92.89$_{0.48}$ (0.64)                                                                 \\
\multicolumn{1}{l|}{\textbf{\pebm-100}} & \textbf{1.89$_{1.06}$}                                           & \textbf{91.94$_{0.14}$}                                                 & \textbf{3.47}                                                    & 168.69$_{0.46}$ (0.64)                                                                \\
\multicolumn{1}{l|}{\textbf{\pebm-150}} & \textbf{1.93$_{1.15}$}                                           & \textbf{91.46$_{0.17}$}                                                 & \textbf{4.14}                                                    & \multicolumn{1}{c}{244.72$_{0.47}$ (0.64)}                                            \\
\multicolumn{1}{l|}{\textbf{\pebm-300}} & \textbf{1.68$_{0.82}$}                                           & \textbf{90.55$_{0.21}$}                                                 & \textbf{2.89}                                                    & \multicolumn{1}{c}{478.29$_{0.47}$ (0.64)}                                            \\ \bottomrule
\vspace{-7mm}
\end{tabular}


==> PureGenDefense/Unused/EBM_training.tex <==

\section{EBM Training}\label{app:ebm_train}

\begin{algorithm}[ht]
\caption{ML with SGD for Convergent Learning of EBM (\ref{eq:ebm})}
\begin{algorithmic}
\REQUIRE ConvNet potential $\mathcal{G}_{\theta}(x)$, number of training steps $J=150000$, initial weight $\theta_1$, training images $\{x^+_i \}_{i=1}^{N_\textrm{data}}$, data perturbation $\tau_\text{data}=0.02$, step size $\tau=0.01$, Langevin steps $T=100$, SGD learning rate $\gamma_\text{SGD}=0.00005$.
\ENSURE Weights $\theta_{J+1}$ for energy $\mathcal{G}_{\theta}(x )$.\\
\STATE
\STATE Set optimizer $g \leftarrow \text{SGD}(\gamma_\text{SGD})$. Initialize persistent image bank as $N_\text{data}$ uniform noise images.
\FOR{$j$=1:($J$+1)}
% \begin{enumerate}
    \STATE 1. Draw batch images $\{x_{(i)}^{+}\}_{i=1}^m$ from training set, where $(i)$  indicates a randomly selected index for sample $i$, and get samples $X_i^+ = x_{(i)} + \tau_\text{data} \epsilon_i$, where i.i.d. $\epsilon_{i} \sim \textrm{N}(0, I_D)$. \\
    \STATE 2. Draw initial negative samples $\{ Y_i^{(0)} \}_{i=1}^m$ from persistent image bank.
    			Update $\{ Y_i^{(0)} \}_{i=1}^m$ with the Langevin equation 
    			\begin{align*}
    			Y^{(k)}_i = Y^{(k-1)}_i -  \Delta \tau \nabla_{Y_{\tau}} f_{\theta_j}(Y_i^{\tau-1})  %\\
       % U(Y^{(k-1)}_i ; \theta_j) 
       + \sqrt{2\Delta\tau} \epsilon_{i, k} ,
                % x_{\tau+1} = x_{\tau} + \Delta \tau \nabla_{x_{\tau}} f_{\theta}(x_{\tau}) + \sqrt{2\Delta \tau} \epsilon_{\tau}  
    			\end{align*}
    			 where $\epsilon_{i , k} \sim \textrm{N}(0, I_D)$ i.i.d., for $K$ steps to obtain samples $\{ X_i^- \}_{i=1}^m = \{ Y_i^{(K)} \}_{i=1}^m$. Update persistent image bank with images $\{ Y_i^{(K)} \}_{i=1}^m$. \\
    \STATE 3. Update the weights by $\theta_{j+1} = \theta_{j} - g(\Delta \theta_j)$, where $g$ is the optimizer and 
    			\[
    			\Delta \theta_j= \frac{\partial}{\partial \theta} \left( \frac{1}{n} \sum_{i=1}^n f_{\theta_j}(X^+_i ) - \frac{1}{m}\sum_{i=1}^m f_{\theta_j}(X_i^-) \right)
    			\]
    			is the ML gradient approximation.
% \end{enumerate}
\ENDFOR
\end{algorithmic}
\label{al:ml_learning}
\end{algorithm}

Algorithm \ref{al:ml_learning} is pseudo-code for the training procedure of a data-initialized convergent EBM. We use the generator architecture of the SNGAN \cite{miyato2018spectral} for our EBM as our network architecture. 

==> PureGenDefense/Unused/archive.tex <==
\section{Archived works.}

\subsection{Experimental Details}

% \begin{table*}[ht!]
%     \centering
%     \caption{Poison success and natural accuracy in all poisoned training scenarios (ResNet18, CIFAR-10). We report the mean and the standard deviations (as subscripts) of 100 GM experiments, 50 BP experiments, and NS triggers over 10 classes. }
%     % First Table
%     \scalebox{0.60}{\input{PureGenDefense/Tables/core_scratch}}
%     % Second Table
%     \scalebox{0.66}{\input{PureGenDefense/Tables/core_transfer}}
%     \label{table:core_results}
% \end{table*}


We compare our method, \pgenEBM, against previous state-of-the-art defenses \epic and \friends  on the current leading triggered poison, Narcissus (NS) and triggerless poisons, Gradient Matching (GM) and Bullseye Polytope (BP). Triggerless attacks GM and BP have 100 and 50 poison scenarios while NS has 10 (one per class). Primary results use a ResNet18 classifier and the CIFAR-10 dataset. We train a variety of EBMs using the training techniques described in App. \ref{sec:ebm_1} with specific datasets for our experimental results:
% $\mathcal{X} \setminus \bigcup_{j=1}^{J} \Pi_j$
\begin{enumerate}
    \itemsep0em 
    \item \textbf{\pgenEBM}: To ensure EBM training is blind to poisoned images, we excluded the indices for all potential poison scenarios which resulted in 37k, 45k, and 48k training samples for GM, NS, and BP respectively of the original 50k CIFAR-10 train images. 
    
    % In this situation, we assume that we have oracle knowledge of which points are being poisoned to mimic a clean In-Distribution dataset, but no knowledge of the poisons or training paradigms themselves.

    \item \textbf{\pgenEBM-P}: Trained on the full CIFAR-10 dataset in which 100\% of training samples are poisoned using their respective class' NS poison trigger. This model explores the ability to learn robust features even when the EBM is exposed to full adversarial influences during training (even beyond the strongest classifier scenario of 10\% poison).

    \item \textbf{\pgenEBM$_{\text{CN-10}}$}: Trained on the CINIC-10 dataset, which is a mix of ImageNet (70k) and CIFAR-10 (20k) images where potential poison samples are removed from CIFAR-10 indices \cite{darlow2018cinic10}. This model investigates the effectiveness of EBM purification when trained on a distributionally similar dataset. 
    % \om{how do u know that it has a similar distribution?} \om{maybe contains the same classes?}

    \item \textbf{\pgenEBM$_{\text{IN}}$}: Trained exclusively on the ImageNet (70k) portion of the CINIC-10 dataset. This model tests the generalizability of the EBM purification process on a public out-of-distribution (POOD) dataset that shares no direct overlap with the classifier's training data $\mathcal{X}$.

    \item \textbf{\pgenEBM-P$_{\text{CN-10}}$}: Trained on the CINIC-10 dataset where the CIFAR-10 subset is fully poisoned. This variant examines the EBM's ability to learn and purify data where a significant portion of the training dataset is adversarially manipulated and the clean images are from a POOD dataset. 
\end{enumerate}

A single hyperparameter grid-search for Langevin dynamics was done on the \pgenEBM model using a single poison scenario per training paradigm (from scratch, transfer linear and transfer fine-tune) as seen in App. \ref{app:grid_search}. The percentage of classifier training data poisoned is indicated next to each poison scenario. Additional details on poison sources, poison crafting, definitions of poison success, and training hyperparameters can be found in App. \ref{app:poison_implement}. 
% \input{PureGenDefense/variable_defs}
\section{EBM Further Background}
\input{PureGenDefense/chaos}


\section{Timing Analysis} \label{app:timing}
Table \ref{table:train_times} shows the training times for each poison defense in the from-scratch scenario on a TPU-V3. As \pgenEBM is a preprocessing step, the purification time ($\sim$400 seconds) is shared across poison scenarios, making it increasingly comparable to no defense as the number of models/scenarios increase. Although EBM training is a compute intensive process, noted in detail in App. \ref{app:ebm_train}, we share results in the section Table \ref{table:core_results} on how a single EBM on a POOD dataset can obtain SoTA performance in a poison/classifier agnostic way. While subset selection methods like \epic can reduce training time in longer scenarios, \pgenEBM offers superior performance and flexibility to the classifier training pipeline. 

\begin{table}[H]
   \centering
   \footnotesize
   \caption{Median Wall Clock Train Times From Scratch}
   \scalebox{0.7}{\input{PureGenDefense/Tables/train_times}}
\end{table}

\section{Additional Model Interpretability Results}

\begin{figure}[H]
    \centering
    \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{PureGenDefense/Figs/captum4.pdf}
    \end{subfigure}
    \vspace{1em} % Space between subfigures

    \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{PureGenDefense/Figs/captum8.pdf}
    \end{subfigure}
    \vspace{1em}

    \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{PureGenDefense/Figs/captum10.pdf}
    \end{subfigure}
    \vspace{1em}

\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{PureGenDefense/Figs/captum12.pdf}
    \end{subfigure}
    \vspace{1em}

    \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{PureGenDefense/Figs/captum22.pdf}
    \end{subfigure}
    \vspace{1em}
        \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{PureGenDefense/Figs/captum24.pdf}
    \end{subfigure}

\end{figure}

\newpage
\subsection{Poisoned Parameters Diverge} 
\cite{yang2022poisons} proposes a subset selection method \epic which rejects poison points through training. 
This defense method produces coresets, that under the PL* condition ($\frac{1}{2}\|\mathbf{\nabla_{\phi }}\mathcal{L}(\phi)\|^{2} \geq \mu\mathcal{L}(\phi), \forall \phi$), when trained on converges to a solution $\phi^*$ with similar training dynamics to that of training on the full dataset. While such a property is attractive for convergence guarantees and preserving the overall performance of the NN, converging with dynamics too close to the poisoned parameters may defeat the purpose of a defense. As such we consider the closeness of a defended network's parameters $\phi^*$ to a poisoned network's parameters $\phi$ by measuring the L1 distance at the end of training ($\left \| \phi-\phi^* \right\|_1$). All distances use the same parameter initialization and are averaged over 8 models from the first 8 classes of the Narcissus poison. In Figure \ref{fig:param_dist_pct}, we specifically consider increasingly higher percentiles of the parameters that moved the furthest away ($\phi_{nth\%},\phi_{nth\%}^*$). The intuition is that poisons impact only a few key parameters significantly that play an incommensurate role at inference time, and hence we would only need to modify a tail of impacted parameters to defend. As we move to increasingly higher percentiles, both the \pgenEBM and \friends defense mechanisms show a greater distance away from the poisoned model weights, indicating significant movement in this long tail of impacted parameters. We find that, as theory predicts, defending with coresets methods yield parameters that are too close to the poisoned parameters $\phi$ leading to sub-optimal defense. 


% Next we consider the parameter distance of each defended model from the poisoned model with no defense at the end of training  with same model initialization, averaging over 8 models from the first 8 classes of the Narcissus poison. In Figure \ref{fig:param_dist_pct}, we specifically consider increasingly higher percentiles of the parameters that moved the furthest away. The intuition is that poisons impact only a few key parameters significantly that play an incommensurate role at inference time, and hence we would only need to modify a long tail of parameters significantly to defend. As we go to increasingly higher percentiles, both the EBM and friendly defense mechanisms show a higher distance away from the poisoned models weights, indicating significant movement in the tail of parameters impacted. Note \epic is a defense that SGD provably converges to a solution $w$ that is within an $\upsilon$-ball of the $w*$ (global minimum of $\mathcal{L}$ ) when SGD is ran on its subsets. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{PureGenDefense/Figs/param_dist_percentiles.pdf}
    \caption{Comparing parameter distances from defended models to poisoned model (same init) for increasingly higher percentiles of the most moved parameters. \pgenEBM trained models show the least movement in the tail of parameter which poisons are theorized to impact most (followed very closely by \friends but well above \epic).}
\end{figure}
\newpage



% \begin{table}[ht]
%    \centering
%    \footnotesize
%    \caption{MobileNetV2 and DenseNet121 architecture results for multiple poison types and training paradigms and HyperlightBench for a novel training paradigm the \pgenEBM can apply to effectively.}
%    \vspace{-2mm}
%    \label{table:model_results}
%    \scalebox{0.68}{\input{PureGenDefense/Tables/models_and_datasets}}
% \end{table}

==> PureGenDefense/Unused/chaos.tex <==
\subsection{Chaotic Dynamics}\label{sec:chaos}
Chaos theory offers a distinct perspective for justifying the suppression of adversarial signals through extended iterative transformations. In deterministic systems, chaos is characterized by the exponential growth of initial infinitesimal perturbations over time, leading to a divergence in the trajectories of closely situated points — a phenomenon popularly known as the butterfly effect. This concept extends seamlessly to stochastic systems as well. \citet{hill2021stochastic} were the first to show the chaotic nature of EBMs for purification. Here we verify that both poisoned images and clean images have the same chaotic properties.

\subsubsection*{Stochastic Differential Equations and Chaos}
Consider the Stochastic Differential Equation (SDE) given by:
\begin{align}
\text{d}X_t = V(X)\text{dt}+ {\eta_{noise}} \text{d}B_t, \label{eqn:sde}
\end{align}
where $B_t$ denotes Brownian motion and ${\eta_{noise}} \ge 0$. This equation, which encompasses the Langevin dynamics, is known to exhibit chaotic behavior in numerous contexts, especially for large values of ${\eta_{noise}}$ \cite{lai2003unstable}.

\subsubsection*{Maximal Lyapunov Exponent}
The degree of chaos in a dynamical system can be quantified by the maximal Lyapunov exponent $\lambda$, defined as:
\begin{align}
\lambda = \lim_{t \rightarrow \infty} \frac{1}{t} \log \frac{|\delta X_{{\eta_{noise}}}(t)|}{|\delta X_{{\eta_{noise}}}(0)|}, \label{eqn:lyapunov}
\end{align}
where $\delta X_{\eta_{noise}} (t)$ represents an infinitesimal perturbation in the system state at time $t$, evolved according to Eq. \ref{eqn:sde} from an initial perturbation $\delta X_{\eta_{noise}} (0)$. For ergodic dynamics, $\lambda$ is independent of the initial perturbation $\delta X_{\eta_{noise}} (0)$. An ordered system exhibits a maximal Lyapunov exponent that is non-positive, while chaotic systems are characterized by a positive $\lambda$. Thus, by analyzing the maximal Lyapunov exponent of the Langevin equation, one can discern whether the dynamics are ordered or chaotic.


Following the classical approach outlined by \citet{benettin1976entropy}, we calculate the maximal Lyapunov exponent for the modified Langevin transformation, described by the equation:
\begin{equation}
Z_{\eta_{noise}} (X)  = x_{\tau} - \Delta \tau \nabla_{x_{\tau}} \mathcal{G}_{\theta}(x_{\tau}) + 
\eta_{noise} \sqrt{2\Delta \tau} \epsilon_{\tau}  ,
\end{equation}

This computation is performed across a range of noise strengths $\eta_{noise}$. 
\begin{figure}[ht] %[H]
    \centering
    \includegraphics[width=.6\textwidth]{PureGenDefense/Figs/lya_exp_results.pdf} \; \includegraphics[width=.2\textwidth]{PureGenDefense/Figs/lya_plot.pdf}
    \caption{\emph{Left:} The maximal Lyapunov exponent varies significantly with different values of the noise parameter $\eta_{noise}$. Notably, at $\eta_{noise}= 1$, which is the setting used in our training and defense dynamics, there is a critical transition observed. This transition is from an ordered region, where the maximal exponent is zero, to a chaotic region characterized by a positive maximal exponent. This observation is crucial for understanding the underlying dynamics of our model. \emph{Right:} The appearance of steady-state samples exhibits marked differences across the spectrum of $\eta_{noise}$ values. For lower values of $\eta_{noise}$, the generated images tend to be oversaturated. Conversely, higher values of $\eta_{noise}$ result in noisy images. However, there exists a narrow window around $\eta_{noise} = 1$ where a balance is achieved between gradient and noise forces, leading to realistic synthesis of images.}
    \label{fig:lya}
\end{figure}
Our findings demonstrate a clear transition from noise-dominated to chaos-dominated behavior. Notably, at $\eta_{noise} = 1$ — the parameter setting for our training and defense algorithms — the system transitions from ordered to chaotic dynamics. This critical interval balances the ordered gradient forces, which encourage pattern formation, against chaotic noise forces that disrupt these patterns. Oversaturation occurs when the gradient forces prevail, leading to noisy images when noise is dominant. These results are illustrated in Figure~\ref{fig:lya}.


The inherent unpredictability in the paths under $Z_{\eta_{noise}}$ serves as an effective defense mechanism against targeted poison attacks. Due to the chaotic nature of the transformation, generating informative attack gradients that can make it through the defense while causing a backdoor in the network becomes challenging.  Exploring other chaotic transformations, both stochastic and deterministic, could be a promising direction for developing new defense strategies.

We see that as expected the Lyapunov exponent of the Langevin dynamics on clean and poisoned points are exactly the same. 

==> PureGenDefense/Unused/variable_defs.tex <==
% \section{To Be Removed}

% \subsection{Variable Definitions (main paper only)}

% \begin{itemize}
%     \item $\Psi(x)$: Stochastic transformation function applied to the input image $x$.
%     \item $x \in \mathbb{R}^D$: Input image or data sample
%     \item $y$: Image label
%     \item $\delta$ and $\rho$: Small adversarial perturbations injected into a fraction of training images. $\delta$ for dataset perturbations, $\rho$ for patch. 
%     \item $\alpha$: The fraction of train images that are poisoned.
%     \item $y^{adv}$: Target label/class for poison method
%     \item $\mathcal{D}$: Dataset of images and labels (test, train); has length $n$. 
%     \item $\mathcal{X}$: Images dataset (test, train)
%     \item $\Pi = \{ (x^\pi , y^\pi) \}$  The set of target image, label pairs
%     \item $F$: Classifier
%     \item $\mathcal{C}$: Set of allowable poisons
%     \item $\eta$: Learning rate
%     \item $\theta$ and $\phi$: Parameters or weights of a model, $\theta$ for EBM, $\phi$ for classifier.
%     % \item $\phi(x)$: 
%     \item $\xi$: Small value representing the magnitude of perturbation in adversarial attacks, often used in the context of crafting adversarial examples.
%     \item $\mathcal{G}(x)$: Energy function in an Energy-Based Model (EBM), where $x$ is the input and $\theta$ represents the parameters of the model.
%     \item $Z$: Partition function, normalizing constant in the context of EBMs.
%     \item $p_{\theta}(x)$: Learned probability distribution function parameterized by $\theta$ in the context of EBMs.
%     \item $L(\theta)$: Loss function with respect to the parameters $\theta$.
%     \item $\nabla L(\theta)$: Gradient of the loss function with respect to the parameters $\theta$.
%     \item $T$: Number of steps in MCMC chain
%     \item $\tau$: Current Step in MCMC chain
%     \item $\gamma$: A parameter, possibly related to the step size in Langevin dynamics or a noise parameter in stochastic processes.
%     \item $X(k)$: State of a system or a sample at step $k$ in Langevin dynamics.
%     \item $\epsilon$: Step size or learning rate parameter, particularly in the context of iterative update rules like Langevin dynamics.
% \end{itemize}

% Appendix

% \begin{itemize}
%     \item $\lambda$: Lyapunov exponent used in the context of chaos theory and dynamical systems.
% \end{itemize}

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer:\answerYes{}%, \answerNo{}, or \answerNA{}.
    \item[] Justification: The claims in the abstract and introduction are supported by the detailed methodologies and comprehensive experimental results presented in Sections \ref{sec:pgen_method} and \ref{sec:experiments}, respectively. These sections demonstrate the effectiveness and universality of \pgen methods in defending against a variety of train-time poisoning attacks. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:\answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations are discussed in Section \ref{sec:limitations}, where we address the computational cost, data requirements for training the generative models, and the trade-offs between purification times and performance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The theoretical results, assumptions, and proofs are detailed in Sections 3.1 and 3.2, with additional mathematical formulations provided in the appendices.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper includes a commitment to release code and models upon publication (along with an anonymous codebase attached for submission). Detailed instructions for reproducing the experiments are provided in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: All relevant training and testing details, including data splits, hyperparameters, and optimizer settings, are thoroughly described in Section 4.1 and Appendix D. The paper includes a commitment to release code and models upon publication (along with an anonymous codebase attached for submission).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Training and test details are, to the best extent of the authors, following previous benchmarks provided by previous poisons authors \cite{poison_baseline, yang2022poisons, zeng2022narcissus, aghakhani2021bullseye}. Otherwise, hyperparameter explanations specific to \pgen{} are given in Section \ref{sec:mcmc_dynamics}. The details of all hyperparameters used are listed in App. \ref{app:training_hyperparams}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The results include error bars in all experiential results in Section \ref{sec:experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Information on the compute resources used, including the type of hardware (TPU V3), memory, and execution time, is provided in Section \ref{sec:limitations} and Table \ref{table:purify_times}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The research adheres to the NeurIPS Code of Ethics, ensuring responsible use of AI technologies and addressing potential ethical concerns related to data poisoning and model security, as discussed in the ``Potential Social Impacts'' Section \ref{app:social}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The social impacts section in App. \ref{app:social} provides a balanced discussion of both positive and negative societal impacts of the research, including ethical considerations and the potential for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The research does not involve the release of high-risk models or datasets that require specific safeguards, but broader risks of the research in general is discussed in Section \ref{app:social}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All datasets and models used are properly cited in Section \ref{sec:experiments} or in Appendix \ref{app:poison_implement}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code and models will be released upon acceptance. Anonymous code is attached with submission. No additional assets. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No Human Subjects
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No Human Subjects
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

